A k-core Decomposition Framework for Graph Clustering

Graph clustering or community detection constitutes an important task for investigating the internal structure of graphs, with a plethora of applications in several domains. Traditional techniques for graph clustering, such as spectral methods, typically suffer from high time and space complexity. In this article, we present CoreCluster, an efficient graph clustering framework based on the concept of graph degeneracy, that can be used along with any known graph clustering algorithm. Our approach capitalizes on processing the graph in an hierarchical manner provided by its core expansion sequence, an ordered partition of the graph into different levels according to the k-core decomposition. Such a partition provides an efficient way to process the graph in an incremental manner that preserves its clustering structure, while making the execution of the chosen clustering algorithm much faster due to the smaller size of the graph's partitions onto which the algorithm operates. An experimental analysis on a multitude of real and synthetic data demonstrates that our approach can be applied to any clustering algorithm accelerating the clustering process, while the quality of the clustering structure is preserved or even improved.

==> Experiments <==
%--------------------------------------------------------------------------
\section{Experimental Evaluation} \label{sec:experiments}
%Begin Figure--------------------------------------------------------------
%%% 3D Figures %%%
\begin{figure}
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/spc/spc_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/spc/spc_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/spc/spc_NMI_D3_3d_plot.eps}
    \caption{Spectral Clustering}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/ifm/ifm_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/ifm/ifm_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/ifm/ifm_NMI_D3_3d_plot.eps}
    \caption{InfoMap}
  \end{subfigure}
  
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/leig/leig_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/leig/leig_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/leig/leig_NMI_D3_3d_plot.eps}
    \caption{Leading Eigenvector}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/fg/fg_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/fg/fg_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/fg/fg_NMI_D3_3d_plot.eps}
    \caption{Fast Greedy}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/mcl/mcl_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/mcl/mcl_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/mcl/mcl_NMI_D3_3d_plot.eps}
    \caption{MCL}
  \end{subfigure}
  \caption{Clustering quality comparisons in terms of NMI for the three artificial graphs (D1, D2, and D3).}
\end{figure}

\begin{figure}
  \ContinuedFloat % continue from previous page
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/metis/metis_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/metis/metis_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/metis/metis_NMI_D3_3d_plot.eps}
    \caption{Metis}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/ml/ml_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/ml/ml_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/ml/ml_NMI_D3_3d_plot.eps}
    \caption{MultiLevel}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/sg/sg_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/sg/sg_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/sg/sg_NMI_D3_3d_plot.eps}
    \caption{SpinGlass}
  \end{subfigure}
  
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/lp/lp_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/lp/lp_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/lp/lp_NMI_D3_3d_plot.eps}
    \caption{Label Propagation}
  \end{subfigure}
  
  \begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[scale=0.24]{3D/wt/wt_NMI_D1_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/wt/wt_NMI_D2_3d_plot.eps}
    \includegraphics[scale=0.24]{3D/wt/wt_NMI_D3_3d_plot.eps}
    \caption{Walktrap}
  \end{subfigure}
  \caption{Continue.... Clustering quality comparisons in terms of NMI for the three artificial graphs (D1, D2, and D3).}
\end{figure}
%End Figure----------------------------------------------------------------

%Begin Figure--------------------------------------------------------------
%%% Facebook Conductance Figures %%%
\begin{figure}
  \begin{subfigure}[b]{1.0\textwidth}
    \centering
    \includegraphics[scale=0.5]{facebook_conductance/conductance_spc.eps}
    \caption{Spectral Clustering}
  \end{subfigure} 
  %  \begin{subfigure}[b]{0.5\textwidth}
  %    \centering
  %    \includegraphics[scale=0.35]{facebook_conductance/conductance_spc.eps}
  %    \caption{Spectral Clustering}
  %  \end{subfigure}
  %  \begin{subfigure}[b]{0.5\textwidth}
  %    \centering
  %    \includegraphics[scale=0.35]{facebook_conductance/conductance_ifm.eps}
  %    \caption{InfoMap}
  %  \end{subfigure}
  
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_leig.eps}
    \caption{Leading Eigenvector}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_fg.eps}
    \caption{Fast Greedy}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_mcl.eps}
    \caption{MCL}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_metis.eps}
    \caption{Metis}
  \end{subfigure}
  \caption{Facebook conductance}
\end{figure}

\begin{figure}
  \ContinuedFloat % continue from previous page
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_ml.eps}
    \caption{MultiLevel}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_sg.eps}
    \caption{SpinGlass}
  \end{subfigure}

  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_ifm.eps}
    \caption{InfoMap}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{facebook_conductance/conductance_wt.eps}
    \caption{Walktrap}
  \end{subfigure}
  \caption{Continue....  Facebook conductance}
\end{figure}
%End Figure----------------------------------------------------------------

%Begin Figure--------------------------------------------------------------
%%% Facebook Time Figures %%%
\begin{figure}
  %\begin{center}
  \begin{subfigure}[b]{1.0\textwidth}
    \centering
    \includegraphics[scale=0.5]{time_fb/spc_time_plot.eps}
    \caption{Spectral Clustering}
  \end{subfigure}
  
  %% \begin{subfigure}[b]{0.5\textwidth}
  %%   \centering
  %%   \includegraphics[scale=0.35]{time_fb/spc_time_plot.eps}
  %%   \caption{Spectral Clustering}
  %% \end{subfigure}
  %% \begin{subfigure}[b]{0.5\textwidth}
  %%   \centering
  %%   \includegraphics[scale=0.35]{time_fb/ifm_time_plot.eps}
  %%   \caption{InfoMap}
  %% \end{subfigure}
  
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/leig_time_plot.eps}
    \caption{Leading Eigenvector}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/fg_time_plot.eps}
    \caption{Fast Greedy}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/mcl_time_plot.eps}
    \caption{MCL}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/metis_time_plot.eps}
    \caption{Metis}
  \end{subfigure} 
  \caption{Facebook time}
\end{figure}

\begin{figure}
  \ContinuedFloat % continue from previous page
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/ml_time_plot.eps}
    \caption{MultiLevel}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/sg_time_plot.eps}
    \caption{SpinGlass}
  \end{subfigure}

  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/ifm_time_plot.eps}
    \caption{Info Map}
  \end{subfigure}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[scale=0.35]{time_fb/wt_time_plot.eps}
    \caption{Walktrap}
  \end{subfigure}
  \caption{Continue.... Facebook time}
\end{figure}
%End Figure----------------------------------------------------------------

==> preamble-jmlr.tex <==
%% Pre-amble - commonly defined macros.

%% Packages

\usepackage{enumerate}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsbsy}
\usepackage{isomath}
%\usepackage{amsthm}
\usepackage{dsfont}
%%\usepackage{theorem}
\usepackage{algorithm}
\usepackage{algorithmic}
%%\usepackage{algpseudocode}
\usepackage{mathrsfs}
\usepackage{paralist}
\usepackage{epsfig}
\usepackage{subfigure}
\usepackage{makeidx} 
\usepackage{color}
\usepackage{hyperref}
%\usepackage{varioref}
\usepackage{tikz}
%\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage{preview}
\usepackage{float}
\usepackage{pgfplots}
\usetikzlibrary{pgfplots.groupplots}
\usetikzlibrary{positioning}

\usepgfplotslibrary{patchplots,colormaps}

%\tikzexternalize
%\usepackage{setspace} %% for using halfspaces

%\usepackage[left=2.5cm,right=2.5cm]{geometry}
%\usepackage[french, english]{babel}

\numberwithin{equation}{section} 

%\theoremstyle{plain} \newtheorem{remark}{Remark}[section]
%%\theoremstyle{plain} \newtheorem{definition}{Definition}[section]
%\theoremstyle{plain} \newtheorem{example}{Example}[section]
%\theoremstyle{plain} \newtheorem{assumption}{Assumption}[section]
%\theoremstyle{plain} \newtheorem{conjecture}{Conjecture}[section]
%\theoremstyle{plain} \newtheorem{theorem}{Theorem}[section]
%\theoremstyle{plain} \newtheorem{proposition}{Proposition}[section]
%\theoremstyle{plain} \newtheorem{lemma}{Lemma}[section]
%\theoremstyle{plain} \newtheorem{corollary}{Corollary}[section]


%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.5em width0.5em depth0.25em\fi}

\newcommand \E {\mathop{\mbox{\ensuremath{\mathbb{E}}}}\nolimits}
\newcommand \hE {\hat{\mathop{\mbox{\ensuremath{\mathbb{E}}}}\nolimits}}
\renewcommand \Pr {\mathop{\mbox{\ensuremath{\mathbb{P}}}}\nolimits}
\newcommand \given {\mathrel{|}}
\newcommand \gvn {|}
\newcommand \eq {{=}}
\newcommand{\set}[1]{\left\{\, #1 \,\right\} }
\newcommand{\cset}[2]{\left\{\, #1 ~\middle|~ #2 \,\right\} }
\newcommand{\meas}[1]{\mu\left(#1\right)}

%% Special characters
\newcommand\Reals {{\mathds{R}}}
\newcommand\Naturals {{\mathds{N}}} 

\newcommand \FB {{\mathfrak{B}}}
\newcommand \FD {{\mathfrak{D}}}
\newcommand \FF {{\mathfrak{F}}}
\newcommand \FM {{\mathfrak{M}}}
\newcommand \FK {{\mathfrak{K}}}
\newcommand \FJ {{\mathfrak{J}}}
\newcommand \FL {{\mathfrak{L}}}
\newcommand \FO {{\mathfrak{O}}}
\newcommand \FS {{\mathfrak{S}}}
\newcommand \FT {{\mathfrak{T}}}
\newcommand \FP {{\mathfrak{P}}}
\newcommand \FR {{\mathfrak{R}}}


\newcommand \CA {{\mathcal{A}}}
\newcommand \CB {{\mathcal{B}}}
\newcommand \CC {{\mathcal{C}}}
\newcommand \CD {{\mathcal{D}}}
\newcommand \CE {{\mathcal{E}}}
\newcommand \CF {{\mathcal{F}}}
\newcommand \CG {{\mathcal{G}}}
\newcommand \CH {{\mathcal{H}}}
\newcommand \CJ {{\mathcal{J}}}
\newcommand \CL {{\mathcal{L}}}
\newcommand \CM {{\mathcal{M}}}
\newcommand \CN {{\mathcal{N}}}
\newcommand \CO {{\mathcal{O}}}
\newcommand \CP {{\mathcal{P}}}
\newcommand \CQ {{\mathcal{Q}}}
\newcommand \CR {{\mathcal{R}}}
\newcommand \CS {{\mathcal{S}}}
\newcommand \CT {{\mathcal{T}}}
\newcommand \CU {{\mathcal{U}}}
\newcommand \CV {{\mathcal{V}}}
\newcommand \CW {{\mathcal{W}}}
\newcommand \CX {{\mathcal{X}}}
\newcommand \CY {{\mathcal{Y}}}
\newcommand \CZ {{\mathcal{Z}}}

\newcommand \BA {{\mathbb{A}}}
\newcommand \BI {{\mathbb{I}}}
\newcommand \BS {{\mathbb{S}}}

\newcommand \bx {{\mathbf{x}}}
\newcommand \by {{\mathbf{y}}}
\newcommand \bu {{\mathbf{u}}}
\newcommand \bw {{\mathbf{w}}}
\newcommand \ba {{\mathbf{a}}}
\newcommand \bat {{\mathbf{a}_t}}
\newcommand \bh {{\mathbf{h}}}
\newcommand \bo {{\mathbf{o}}}
\newcommand \bp {{\mathbf{p}}}
\newcommand \bs {{\mathbf{s}}}
\newcommand \br {{\mathbf{r}}}

\newcommand \SA {\mathscr{A}}
\newcommand \SB {\mathscr{B}}
\newcommand \SC {\mathscr{C}}
\newcommand \SF {\mathscr{F}}
\newcommand \SG {\mathscr{G}}
\newcommand \SH {\mathscr{H}}
\newcommand \SJ {\mathscr{J}}
\newcommand \SL {\mathscr{L}}
\newcommand \SP {\mathscr{P}}
%%\newcommand \SS {\mathscr{S}}
\newcommand \ST {\mathscr{T}}
\newcommand \SU {\mathscr{U}}
\newcommand \SV {\mathscr{V}}
\newcommand \SW {\mathscr{W}}

\newcommand \hM {\widehat{M}}

\newcommand \p {\partial}

\newcommand \then{\Rightarrow}
\newcommand \defn {\mathrel{\triangleq}}
%\newcommand \StateSet {{\CQ}}


%% Commands

\newcommand \argmax{\mathop{\rm arg\,max}}
\newcommand \argmin{\mathop{\rm arg\,min}}
\newcommand \dtan{\mathop{\rm dtan}}
\newcommand \sgn{\mathop{\rm sgn}}
\newcommand \trace{\mathop{\rm tr}}

\newcommand \onenorm[1]{\left\|#1\right\|_1}
\newcommand \pnorm[2]{\left\|#1\right\|_{#2}}
\newcommand \inftynorm[1]{\left\right\|#1\|_\infty}
\newcommand \norm[1]{\left\|#1\right\|}

%%\newcommand \defn {\triangleq}
%%\newcommand \defn {\equiv}
%%\newcommand \defn {\coloneq}
%%\newcommand \defn {\stackrel{\text{\tiny def}}{=}}
%%\newcommand \defn {\stackrel{\text{def}}{\hbox{\equalsfill}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand \Normal {\mathop{\mathpzc{N}}\nolimits}
\newcommand \Wishart {\mathop{\mathpzc{W}}\nolimits}
\newcommand \Poisson {\mathop{\mathpzc{Poisson}}\nolimits}
\newcommand \Multinomial {\mathop{\mathpzc{Multinomial}}\nolimits}
\newcommand \Dirichlet {\mathop{\mathpzc{Dirichlet}}\nolimits}
\newcommand \Student {\mathop{\mathpzc{Student}}\nolimits}
\newcommand \Bernoulli {\mathop{\mathpzc{Bernoulli}}\nolimits}
\newcommand \Beta {\mathop{\mathpzc{Beta}}\nolimits}
\newcommand \GammaDist {\mathop{\mathpzc{Gamma}}\nolimits}
\newcommand \Softmax{\mathop{\mathpzc{Softmax}}\nolimits}
\newcommand \Exp{\mathop{\mathpzc{Exp}}\nolimits}
\newcommand \Uniform{\mathop{\mathpzc{Unif}}\nolimits}

\newcommand \Beliefs {\Xi}
\newcommand \Actions {\CA}
\newcommand \States {\CS}

\newcommand \Borel[1] {\FF(#1)}
\newcommand \Probs[1] {\FM(#1)}

\newcommand \pol {\pi}
\newcommand \Pols {\Pi}
\newcommand \mdp {\mu}
\newcommand \MDPs {\CM}
\newcommand \meanMDP {{\bar{\mdp}_\xi}}

\newcommand {\msqr} {\vrule height0.33cm width0.44cm}
\newcommand {\bsqr} {\vrule height0.55cm width0.66cm}

\newcommand\ind[1]{\mathop{\mbox{\ensuremath{\mathbb{I}}}}\left\{#1\right\}}
\newcommand\Ind{\mbox{\bf{I}}}

\newcommand\dd{\,\mathrm{d}}

\newcommand \seq[2]{#1^{#2}}
\newcommand \pseq[3]{#1_{#2}^{#3}}
\newcommand \sam[2]{#1^{(#2)}}

\newcommand \eye {\matrixsym{I}}
\newcommand \MA {\matrixsym{A}}
\newcommand \MX {\matrixsym{X}}
\newcommand \MY {\matrixsym{Y}}
\newcommand \MB {\matrixsym{B}}
\newcommand \MV {\matrixsym{V}}
\newcommand \MW {\matrixsym{W}}
\newcommand \MP {\matrixsym{P}}
\newcommand \vs {\vectorsym{s}}
\newcommand \vx {\vectorsym{x}}
\newcommand \vq {\vectorsym{q}}
\newcommand \vz {\vectorsym{z}}
\newcommand \vr {\vectorsym{r}}
\newcommand \vm {\vectorsym{m}}
\newcommand \vb {\vectorsym{b}}
\newcommand \vt {\vectorsym{\theta}}

\newcommand \pn[1] {\vz_{[#1]}}

\newcommand \ctx {f}
\newcommand \basis {\phi}
\newcommand \bel {p}
\newcommand \mbel {\Normal}
\newcommand \pbel {\Wishart}

\newcommand \pmean {\matrixsym{M}}
\newcommand \pcov {\matrixsym{C}}
\newcommand \pwish {\matrixsym{W}}
\newcommand \porder {n}

\newcommand \Syx {\matrixsym{\Sigma}_{yx}}
\newcommand \Sxx {\matrixsym{\Sigma}_{xx}}
\newcommand \Syy {\matrixsym{\Sigma}_{yy}}
\newcommand \Symx {\matrixsym{\Sigma}_{y\mid x}}

\newcommand \trans[1] {#1^\top}

\newcommand \noise {\vectorsym{\varepsilon}}

\newcommand \node[1] {\nu_{#1}}
\newcommand \pt {p_t}


\newcommand \CSet {G}
\newcommand \RSet {\hat{G}}
\newcommand \Parent[1] {\mathfrak{P}(#1)}
\newcommand \Children[1] {\mathfrak{C}(#1)}
\newcommand \Ancestors[1] {\mathfrak{A}(#1)}
\newcommand \Descendants[1] {\mathfrak{D}_t(#1)}
\newcommand \metric[2] {\psi(#1, #2)}
\newcommand \zooming {\zeta}
\newcommand \depth[1] {d(#1)}
\newcommand \level[1] {\ell(#1)}
\newcommand \kLSTD {K_{\textrm{L}}}

\newcommand \kAPI {K_{A}}
\newcommand \dimS {m}
\newcommand \dimLSTD {m_L}
\newcommand \nsam {n_{s}}
\newcommand \ntraj {n_{\text tr}}
\newcommand \Ttraj {T_{\text tr}}

\newcommand \disc {\gamma}
\newcommand \rew {\rho}

\newcommand{\errorband}[5][]{ % x column, y column, error column, optional argument for setting style of the area plot
\pgfplotstableread[col sep=comma, skip first n=2]{#2}\datatable
    % Lower bound (invisible plot)
    \addplot [draw=none, stack plots=y, forget plot] table [
        x={#3},
        y expr=\thisrow{#4}-\thisrow{#5}
    ] {\datatable};

    % Stack twice the error, draw as area plot
    \addplot [draw=none, fill=gray!40, stack plots=y, area legend, #1] table [
        x={#3},
        y expr=2*\thisrow{#5}
    ] {\datatable} \closedcycle;

    % Reset stack using invisible plot
    \addplot [forget plot, stack plots=y,draw=none] table [x={#3}, y expr=-(\thisrow{#4}+\thisrow{#5})] {\datatable};
}


%%% macros to make things smalller
% For comparison, the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{%
           \llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{%
           \rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{%
           \clap{$\mathsurround=0pt#1{#2}$}}


\usetikzlibrary{automata}
\usetikzlibrary{topaths}

\tikzstyle{select}=[rectangle,draw=black,fill=red!20,inner sep=0mm, minimum size=9mm]
\tikzstyle{hidden}=[circle,dashed,draw=black,fill=green!20,inner sep=0mm, minimum size=9mm]
\tikzstyle{observed}=[circle,draw=black,fill=blue!10,inner sep=0mm, minimum size=9mm]







